Asynchronous Implementation of Failure Detectors with partial connectivity and unknown participants

We consider the problem of failure detection in dynamic networks such as MANETs. Unreliable failure detectors are classical mechanisms which provide information about process failures. However, most of current implementations consider that the network is fully connected and that the initial number of nodes of the system is known. This assumption is not applicable to dynamic environments. Furthermore, such implementations are usually timer-based while in dynamic networks there is no upper bound for communication delays since nodes can move. This paper presents an asynchronous implementation of a failure detector for unknown and mobile networks. Our approach does not rely on timers and neither the composition nor the number of nodes in the system are known. We prove that our algorithm can implement failure detectors of class <>S when behavioral properties and connectivity conditions are satisfied by the underlying system.

==> abstract.tex <==
We consider the problem of failure detection in dynamic network such
as MANET  Unreliable failure detectors (FD) are classical mechanisms
providing information about process failures. They allow to solve
consensus in asynchronous network. However, most of implementations
consider a set of known processes fully connected by reliable links.
Such an assumption is not applicable in dynamic environments.
Furthermore, the majority of current failure detector implementation
are timer-based ones while in dynamic networks there is not an upper
bound for communication delays. This paper presents an asynchronous
implementation of a failure detector for dynamic environments. Our
implementation is an extension of the query-response algorithm
previously proposed by Mostefaoui, Mourgaya and Raynal
\cite{mostefaoui03async} which does not rely on timers to detect
failures. We assume that neither the identity nor the number of
nodes are initially known.  We also proof that our algorithm can
implement failure detectors of class $\diamondsuit S$ when some
behavioral properties are satisfied by the underlying system.
Simulation results have validated our approach.

